Tunable and Portable Extreme-Scale Drug Discovery Platform at Exascale: the LIGATE Approach

Today digital revolution is having a dramatic impact on the pharmaceutical industry and the entire healthcare system. The implementation of machine learning, extreme-scale computer simulations, and big data analytics in the drug design and development process offers an excellent opportunity to lower the risk of investment and reduce the time to the patient. Within the LIGATE project, we aim to integrate, extend, and co-design best-in-class European components to design Computer-Aided Drug Design (CADD) solutions exploiting today's high-end supercomputers and tomorrow's Exascale resources, fostering European competitiveness in the field. The proposed LIGATE solution is a fully integrated workflow that enables to deliver the result of a virtual screening campaign for drug discovery with the highest speed along with the highest accuracy. The full automation of the solution and the possibility to run it on multiple supercomputing centers at once permit to run an extreme scale in silico drug discovery campaign in few days to respond promptly for example to a worldwide pandemic crisis.

==> CF23_LIGATE (2)/DOCKaaS.tex <==
\subsection{Virtual Screening-as-a-Service.}
Among the several goals, LIGATE directly addresses the contemporary challenges that running a virtual screening campaign at a large scale requires extensive expertise and manual intervention. This is motivated by the fact that (i) there is a lack of ability for different tools to interoperate efficiently and automatically through APIs and well-specified data formats, and (ii) that the efficient management of large HPC resources requires additional skills that are not always available for domain experts.

To address this issue, we integrated the LiGen molecular docking application with an HPC-as-a-Service framework (HEAppE \footnote{HEAppE Website - \url{https://heappe.eu/web}}) \cite{Svaton2020280} to permit the execution of virtual screening tasks on supercomputing resources through REST API without a direct access to them. This allowed us the simple integration with the LEXIS Platform \cite{Golasowski202217} which provides an easy to use web-portal to manage data and workflow execution on remote HPC resources.

The LEXIS platform and the integrated LiGen-related workflow have been designed to enable multi-site execution of a large-scale computation in case of urgent computing, thus permitting the deployment of part of the virtual screening campaign on multiple HPC centers without the need for explicit management. A central part of this platform is the support for distributed data management between different sites together with data staging to/from HPC resources. 
%
The LEXIS-LiGen integration permits also to envision the use of the LIGATE platform at the end of the project in a Virtual Screening-as-a-service fashion for researchers and public institutions.
%Another benefit of this solution is a specialised portal which is providing easy access to the capabilities of the supercomputing systems for users who do not necessarily have deep experience with them.

==> CF23_LIGATE (2)/DataAware.tex <==
%\subsection{Data-aware high-throughput computing pattern} 

In addition to the parameters that are explicitly exposed by LiGen, we also exploited the possibility of auto-tune part of the code according to the characteristics of the input data, i.e. the ligands.
In fact, to target high-throughput experiments making better use of GPUs, we completely re-designed LiGen in a way that it processes a \emph{batch} of ligand-protein pairs across the device, instead of a single one as done by state-of-the-art approaches \cite{10.48550/arxiv.2209.05069}. 
To maximize the efficiency of the new approach the ligands are clustered by size before the GPU kernels and are temporarily stored in a set of buffers. The GPU computation is launched once one of the batches reached a specific size that is dependent on the ligand characteristics, i.e. number of atoms and rotatable bonds, and GPU memory/micro-architecture.
The fine-grain tuning of the batch size for each ligand size has been derived using an abstract model of the device that resulted to be portable across the different analyzed GPUs.

%However, this implementation requires a fine-grain tuning of the size of the batch to be processed that strongly depends on the ligand size, i.e. number of atoms and rotatable bonds.


%We also explored the impact of a data preparation phase that uses input and architecture (GPU) features to improve computation efficiency.

==> CF23_LIGATE (2)/HQ.tex <==
\subsection{Efficient sub-node task scheduler.} Modern HPC clusters contain a large number of heterogeneous resources that provide vast amounts of computational power. The potential of these clusters might not be fully exploited when users submit a large number of tasks that cannot utilize the whole computational node. Existing HPC job managers are not well prepared for such scenarios, which can lead to nodes being underutilized.

HyperQueue is a task runtime framework \footnote{https://github.com/It4innovations/hyperqueue} designed for the efficient execution of a large number of heterogeneous tasks on HPC systems, which was developed within LIGATE. It takes care of asking for computational resources from the job manager on behalf of the user, and load balances submitted tasks on all available computing nodes with a sophisticated scheduler to keep node utilization as high as possible.

HyperQueue has been used within LIGATE to simplify the execution of the target in-silico virtual screening application, which is composed of many small tasks. Using HyperQueue, users of the application do not have to care about splitting the tasks into individual HPC jobs and then submitting these jobs separately. They simply submit all tasks into HyperQueue and it takes care of the rest.


==> CF23_LIGATE (2)/ML_WP4.tex <==

\subsection{Machine Learning engines to further speedup the virtual screening phase}
In LIGATE, we want to exploit the possibility of generating a large set of data to analyze the possibility to use Machine Learning (ML) techniques to further speed up the virtual screening phase. In particular, one of the goals of the project is to evaluate the possibility of predicting the binding affinity in the early stages of the CADD platform, using the costly free energy computation derived by GROMACS as ground truth. 
%As an example, the prediction algorithms based on machine learning techniques will be used to rank the most promising poses or to directly filter out unpromising ligands. 

Since the design of the best prediction algorithm for a given class of applications strictly depends on the problem at hand and on the available data, this task will evaluate different machine learning approaches starting from simple, computationally efficient techniques (e.g. multivariate regressions) up to techniques demanding more computational effort, such as deep/graph neural networks. 
The most suitable prediction technique for the CADD platform has to be identified considering the cost to obtain the prediction in relation to the specific usage of the CADD platform. 
Fast screening of a large ligand database (e.g. in case of urgent computing) would require a cheaper prediction model, while a more detailed analysis on a reduced set of molecules can use a more computationally demanding model. Starting from the scoring function already available in LiGen \cite{beccari2013ligen}, we will identify the features related to ligand, pocket and their interaction to be used as input variables of the free-energy prediction model to be used. Moreover, we are going to analyze the possible subset of them that can be used also to steer the pose generation during the geometric docking phase \cite{gadioli2021tunable} which is the core engine within LiGen.

While waiting for the data to be generated by free energy calculations on GROMACS, we analyzed the problem of pose selection. Pose selection is the step within the structure-based virtual screening phase that is in charge of the selection of the most reliable and interesting poses to be evaluated in terms of binding affinity. We generated a large set of data using LiGen and we labeled them using the RMSD with respect to known experimental poses. Several state-of-the-art machine learning methods have been analyzed while looking at the most promising ones. 3D-CNN (Convolutional Neural Networks, i.e. Pafnucy \cite{3DCNN}, and DimeNet \cite{dimenet}), GNN (Graph Neural Networks, i.e. GraphBar \cite{graphbar}), and MDN (Mixture Density Network, i.e. DeepDock \cite{DeepDock}, and RTMScore \cite{rtmscore}) have been retrained using the generated large set of RMSD labeled data and are currently under investigation for a seamless integration within the pipeline. 

Moreover, a novel pose selector scheme called LiHPS (LiGen High-throughput Pose Selector), targeting extreme-scale virtual screening campaigns, has been developed from scratch adopting a mix of approximate computing, and supervised/unsupervised techniques. With respect to the previously mentioned 3D-CNN/GNN/MDN methods, LiHPS exploits another sweet spot in the throughput-accuracy trade-off curve, where a small reduction in accuracy brings a very large performance improvement.


==> CF23_LIGATE (2)/PerfPort.tex <==
\subsection{Performance Portability} 
Modern high-performance computing (HPC) systems leverage hardware heterogeneity (e.g. GPUs, FPGAs) as a key feature. 
%These systems are typically composed of central processing units (CPUs) along with multiple accelerators such as graphics processing units (GPUs), field-programmable gate arrays (FPGAs), and application-specific integrated circuits (ASICs) to offload computationally-intensive and domain-specific tasks. 
In the HPC scenario, the Top500 list \footnote{Top500 List Website - \url{https://www.top500.org/}} shows that, at the end of 2022, eight out of the ten top systems are GPU-accelerated, with NVIDIA and AMD being the primary hardware providers. 
However, applications developed for GPUs are often written in proprietary, non-portable programming languages, such as CUDA for NVIDIA GPUs, which can lead to vendor lock-in and hinder the ability to quickly migrate to different platforms. Moreover, being bound to a single architecture can significantly impact the application's ability to be applied in urgent computing scenarios where the maximum computing power needs to be harnessed. Therefore, it is crucial to have application code that can efficiently run on different devices. 

In recent years, several programming models for heterogeneous computing have been proposed. One such model is SYCL\cite{SYCL2020}, a royalty-free, cross-platform abstraction layer that enables code for heterogeneous processors to be written using standard ISO C++. SYCL allows for both the host and kernel code for an application to be in the same source file. The Kronos Group consortium maintains SYCL, and it has multiple implementations provided by companies, such as Intel \cite{oneapi}, and universities \cite{opensycl}. SYCL enables the development of high-level, performance-portable applications that can target CPUs, GPUs, and FPGA cards without requiring device-specific code.

Within LIGATE, we designed a \textit{performance-portable} implementation of LiGen, originally written in C++ and CUDA to target only NVIDIA GPUs \cite{9817028, vitali2019exploiting}. We ported the legacy code to SYCL2020 analyzing different alternative possibilities (e.g., adopting Unified Shared Memory and Buffer-Accessors paradigms). The new SYCL implementation can target CPUs, as well as both NVIDIA and AMD GPUs, unlocking the possibility to run on the GPU partition of LUMI supercomputer and on an E4 internal research cluster.

Figure \ref{fig:LigBench} presents the performance results in terms of Ligands per second per GPU  with both the native CUDA application and the SYCL version. While the former can only run on NVIDIA hardware, for the SYCL version we show the results on both NVIDIA (A100, V100) and AMD (MI250X, MI100) GPUs using the OpenAPI and OpenSYCL compilers. The results have been benchmarked on three top European supercomputers, and on the E4 research cluster.
%
While the native CUDA version achieves a higher throughput on the same hardware, the SYCL version is able to run also on AMD GPUs with comparable performance, while also proving a ground base for following optimizations tailored to novel systems (e.g. LUMI cluster).

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/LigenBench.pdf}
    \caption{LiGen Performance Results on different Clusters (IT4I-Karolina, CINECA-Marconi100, LUMI-G and E4), and using different implementations (CUDA and SYCL)and software stacks (OpenSYCL, OneAPI). }
    \label{fig:LigBench}
    %\vspace{7pt}
\end{figure}

\subsection{The Celerity Runtime System}
While SYCL aids in alleviating the portability issues of single-GPU code across vendors, developers of applications targeting a distributed memory cluster with accelerators still have to contend with manually implementing communication. Doing so efficiently, especially in the presence of the large amount of low-level details introduced by GPU computing and network communication across different vendors, topologies, and technology stacks, is a challenge even for parallel system experts. % Furthermore, a low-level implementation e.g. in MPI will by necessity encode algorithmic decisions in its communication implementation, making it more difficult to explore other options.
%
The Celerity Runtime System~\cite{salzmann2023async} provides a high-level C++ layer closely inspired by SYCL, which automatically manages work distribution and data dependencies. It enables high-productivity development of applications for GPU clusters~\cite{thoman2019celerity}, only requiring efforts comparable to a baseline single-GPU SYCL implementation.

Within the LIGATE project, we have extended the Celerity system with new high-level primitives to more directly encode the semantics of the target applications~\cite{thoman2022celerity}, and we improved the throughput on large systems by introducing a zero-communication-overhead distributed command generation scheme~\cite{salzmann2023async}.



\subsection{LiGen Autotuning}

In the context of HPC, autotuning \cite{autotuningHPC, antarex} refers to the process of automatically selecting the best configuration of the software or compiler parameters according to a specific target hardware and execution condition. This automatic process permits a more efficient execution of the code eliminating the need for manual intervention. 
The importance of autotuning is not only for a specific application-architecture pair, but it has a huge impact when it is important to guarantee performance portability across multiple architectures or application versions that can exploit a different best configuration. 

Several autotuning software solutions exist \cite{ansel2014opentuner, gadioli} that allow to efficiently explore the configuration space with varying degrees of complexity, with or without the possibility of taking constraints into account. %OpenTuner \cite{}, Optuna \cite{akiba2019optuna}, , are only some examples of autotuning tools that are available from literature.
%
Within LIGATE, our intention has been to exploit this possibility together with an explicit parameterization of one of the main LIGATE components.
In particular, we revised the original LiGen code by exposing as much as possible the internal parameters that can have an impact on both quality and performance, or that can spot different optimization opportunities on different architectures. 
We extracted 11 software parameters (knobs) of the LiGen application, accounting for overall more than 60 million different configurations, and we run a tuning campaign to search for Quality-Performance tradeoffs.
The importance of the trade-off is the possibility to use the same docking tool for both small-scale campaigns requiring higher quality, and extreme-scale virtual screening experiments where the overall duration of the campaign and resource usage (cost) can be the actual limit.
To make the exploration feasible from the execution time perspective, we adopted an iterative approach based on the Bayesian Optimization (BO) algorithm supported by Machine Learning techniques, named MALIBOO \cite{guindani2022maliboo}. This approach is efficient in minimizing the execution costs of recurring resource-constrained computing jobs.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/Tuning2.pdf}
    \caption{Exploration of the LiGen software knob}
    \label{fig:LigEXPLORE}
    %\vspace{7pt}
\end{figure}

Figure \ref{fig:LigEXPLORE} shows an example of the exploration results where obtained evaluating a small subset of 320 different LiGen configurations (blue dots). In particular, the RMSD (Root Mean Square Distance) calculation refers to the distance between the predicted best pose and the actual experimental pose for each ligand-protein pair derived from the CASF2016 dataset \cite{CASF16}. The wall-time refers to the overall time needed to screen 1M ligands.






==> CF23_LIGATE (2)/Ph3App.tex <==
\subsection{Key Technologies on the Cronos Use Case}
To further validate the technology developed to support the tuning, parallelization, and portability of the CADD platform for extreme-scale virtual screening, within the project an additional use case has been considered. 
%
The selected application, Cronos~\cite{kissmann2018cronos}, comes from the astro- and particle physics world, a completely different field with respect to LiGen and GROMACS. A structured grid magneto-hydrodynamics simulation in 3D that resolves plasma-dynamical problems in astrophysics and space science. 
%It is most frequently used for computing gamma-ray emissions of binary star system LS 5039, with a decent amount of performance and scalability data available.
%
The original implementation is written in C++, and parallelized using MPI to target CPU-based distributed memory systems. %, and was successfully used in a PRACE Access project. 
This version, while demonstrating excellent scalability on medium-sized clusters (approx.\ 95\% parallel efficiency on 1024 cores, 60-70\% on 16,384 cores), does not use GPUs despite the fact that structured grid applications are often well-suited for accelerated clusters.

The goal for Cronos within LIGATE is (1) to have a SYCL and Celerity~\cite{salzmann2023async} implementation to enable a portable GPU execution, (2) to rigorously test both platform suitability for this use case as well as performance and scalability, and (3) to investigate and benchmark possible performance optimizations.
%\textbf{Current achievements.}
At the current stage of the project, a functional SYCL porting is available. A deviation in the output from the CPU to GPU execution originates from the different implementations of reduction algorithms coupled with floating-point math semantics. The Celerity implementation is ongoing, after which initial performance tests can be performed to drive further optimization work.


==> CF23_LIGATE (2)/WP5.tex <==
\subsection{Scientific validation of the CADD platform}

The LIGATE CADD platform is a promising tool for structure-based drug discovery due to its key characteristics: portability, tunability, and scalability. 
 However, we plan to demonstrate the effectiveness of the technology not only by considering extra-functional aspects but also analyzing the actual advantages that the innovative CADD platform can bring to the target drug discovery field.

To do so, we have compiled comprehensive datasets of protein-ligand complexes that encompass a diverse range of drug targets and small molecules. These benchmark datasets are derived from the PDB and meet rigorous quality criteria, serving as a reliable "ground truth" for the evaluation of the LIGATE CADD platform. We have ensured the diversity of the datasets from three perspectives: protein, ligand, and binding pocket, ensuring sufficient representation of each. Moreover, we have included special sets of mutant structures and similar ligands to better assess the platform's performance in challenging cases. We then developed an automated pipeline for continuous benchmarking and evaluation of the virtual screening platform, with automated reporting on the scale and areas of improvement.

%As a next step, we collaborate with the National Center for Competence in Research in Antimicrobial resistance (NCCR Antiresist) at the University of Basel and select antimicrobial drug targets for infectious diseases as real world test cases. \textit{In vitro} experimental validation of hits identified by the CADD platform would demonstrate the practical applicability of the approach on disease targets with high medical relevance according to the WHO priorities.
As the final step, the project consortium plan to select antimicrobial drug targets for infectious diseases as real-world test cases. \textit{In vitro} experimental validation of hits identified by the CADD platform would demonstrate the practical applicability of the approach on disease targets with high medical relevance according to the WHO priorities. 
%
The results will be published in peer-reviewed journals, and benchmark data will be made openly accessible under FAIR data principles.

%\textbf


==> CF23_LIGATE (2)/gromacs.tex <==
\subsection{Integrated automatic setup and execution of free energy calculations}

The main goal of the molecular simulation work in LIGATE is to provide
a high-performance implementation of accurate free energy calculations that is
also fully automated and portable. To achieve this, we have first developed a workflow ranking drug candidates by their relative free energy of binding (RBFE) to the target protein. Starting from lists of thousands of docked compounds/poses, this workflow with its new interfaces can automatically determine the force field parameters for both the protein and the compound, set up free energy calculations in GROMACS, execute the entire ensemble as a parallel run on HPC resources using HyperQueue (See Section 3.6), and return free energies with a requested standard error. 

To obtain the RBFE estimates with a minimal number of molecular dynamics (MD) steps, the compounds are grouped into pairs that are alchemically transformed into each other during the MD simulations, which requires the workflow to solve the maximum common substructure problem for each compound pair. In the MD simulations, the Accelerated Weight Histogram method (AWH) creates a bias potential to facilitate the alchemical transformation of the compound pair, and this bias potential converges to the RBFE.~\cite{Lundborg2021}. For GROMACS-2023, the performance of free energy calculations has also been improved by rewriting the 
free energy non-bonded kernels to use SIMD instructions, which more than doubles
performance when the algorithm is a bottleneck, which was typically the case when running e.g. on GPU accelerators.

Finally, to build an AI engine supporting the analysis in the early stages of the CADD platform, it is necessary to go beyond relative free energies and rather target 
absolute binding free energies (ABFEs) of protein-compound complexes. To this end, we are developing a variant of the above workflow in which the free energy calculations are replaced with standard MD simulations with GROMACS. ABFEs are subsequently estimated from the MD trajectories as the sum of gas and solvation free energy with gmx\_MMPBSA.~\cite{ValdesTresanco2021}

% The ASMESIS-SV workflow is the workflow needed to calculate ABFEs
% Although describing it, I deliberately avoided using the name
% because the acronym was chosen before the actual usecase and 
% some technical details were clear. Therefore, the acronym is no longer
% correct and has to be updated in the future.
